Distribution learning via neural differential equations: a nonparametric statistical perspective

Ordinary differential equations (ODEs), via their induced flow maps, provide a powerful framework to parameterize invertible transformations for the purpose of representing complex probability distributions. While such models have achieved enormous success in machine learning, particularly for generative modeling and density estimation, little is known about their statistical properties. This work establishes the first general nonparametric statistical convergence analysis for distribution learning via ODE models trained through likelihood maximization. We first prove a convergence theorem applicable to arbitrary velocity field classes $\mathcal{F}$ satisfying certain simple boundary constraints. This general result captures the trade-off between approximation error (`bias') and the complexity of the ODE model (`variance'). We show that the latter can be quantified via the $C^1$-metric entropy of the class $\mathcal F$. We then apply this general framework to the setting of $C^k$-smooth target densities, and establish nearly minimax-optimal convergence rates for two relevant velocity field classes $\mathcal F$: $C^k$ functions and neural networks. The latter is the practically important case of neural ODEs. Our proof techniques require a careful synthesis of (i) analytical stability results for ODEs, (ii) classical theory for sieved M-estimators, and (iii) recent results on approximation rates and metric entropies of neural network classes. The results also provide theoretical insight on how the choice of velocity field class, and the dependence of this choice on sample size $n$ (e.g., the scaling of width, depth, and sparsity of neural network classes), impacts statistical performance.

==> OLD-CK-PROOFS.tex <==


\section{Remaining proofs for Section \ref{Ck-theory}}

\begin{proof}[Proof of Theorem \ref{Thm:existencCkField}]
The first part of the theorem follows from results in \cite{FirstPaper}. It therefore remains to prove the second claim, whose proof we break into three steps.
	
\paragraph{Step 1: $T$ vanishes linearly near the boundary}
	
    Let $i\in\{1,2,...,d\}$ be any coordinate. We will show that there exists $\epsilon > 0$ such that for all $x_i\leq \epsilon$, $T_i(x_1,..,x_i) = c_i(x_1,...,x_{i-1})x_i$ for some function $c_i\in C^k([0,1]^{i-1})$. Moreover, for $x_i\in[1-\epsilon, 1]$, $T_i(x_1,...x_i) = 1 - (1-x_i)\tilde{c}(x_1,...,x_{i-1})$ for another function $\tilde{c}_i\in C^k([0,1]^{i-1})$. \todo{How about the $1$-boundary? We need to say something about it.}
	
	Recall that for the KR map that pushes forward $P_0$ to $\rho$, it holds that $$T_i(x_1,...,x_i) = F_{\rho, i}(T_1(x_1),...,T_{i-1}(x_{[i-1]}), \cdot)^{-1}\circ F_{P_0, i}(x_{[i]}),$$
	where
	\[F_{P_0, i}(x_{[i]}) = \frac 1{\tilde{p}_{0, i-1}(x_{[i-1]})} \int_0^{x_i}\tilde{p}_{0,i}(x_{[i-1]}, y)dy\]
	is the marginal cdf of $x_i$ conditional on $x_{[i-1]}$. Here, $\tilde{p}_{0, i-1}$ and $\tilde{p}_{0, i}$ are the marginal densities of $x_{[i-1]}$ and $x_i$ respectively.
	
	Under the assumption that $p_0\in \mathcal M(k,L_1,L_2)$, we know that $p_0\equiv 1$ on $D\setminus \mathcal O$. Since we assumed that $\bar O \subseteq (0,1)^d$, there exists some $\epsilon$ such that for all $x\in \bar O$, $\textnormal{dist}(x,\partial D)>\eps$. Thus, if either $x_i \in [0, \epsilon)$ or $x_i\in [1-\eps, 1]$, then necessarily $x\ne \mathcal O$. Now let us assume that $x_i \in [0, \epsilon)$ and prove the first assertion; the proof of the second assertion for $x_i\in [1-\eps, 1]$ is the same.
	
	Since $\inf_{z\in\mathcal O}\textnormal{dist}(z,\partial D)>\eps$, it is clear that for any $y\le x_i$, $\tilde{p}_{0,i}(x_{[i-1]}, y)  = 1.$ Consequently, it follows that \[F_{P_0, i}(x_{[i]}) = \frac 1{\tilde{p}_{0, i-1}(x_{[i-1]})} \int_0^{x_i}\tilde{p}_{0,i}(x_{[i-1]}, y)dy= \frac{x_i}{\tilde{p}_{0, i-1}(x_{[i-1]})}.\] 
	
	
	
	Moreover, we have that the marginal densities satisfies $\tilde {p}_{0, i-1}\in C^k([0,1]^{i-1})$, as well as the lower bound $\tilde{p}_{0, i-1}\in C^k([0,1]^{i-1}) \geq L_2$. It thus follows that $x\mapsto \frac{1}{\tilde{p}_{0, i-1}(x_{[i-1]})}\in C^k([0,1]^{i-1})$, and the claim follows.
	
	
	
	
\paragraph{Step 2: $f_{p_0}^\Delta$ vanishes linearly near the boundary}
	
	Note $G$ from (\ref{eq: G}) is triangular in the first $d$-components. Write 
	$$G(x_1,...x_d,t) = [G_1(x_1,t),...,G_d(x_1,...,x_d,t)]^T,$$
	where $G_i(x_1,...,x_i, t) = tT_i(x_1,...,x_i) + (1-t)x_i$. 
	
	By the construction of KR map, we know the inverse of the $i-$th component conditioned on the first $i-1$ components, denoted by $T_i^{-1}[x_1,...,x_{i-1}](x_i)$,  is well-defined. Furthermore, conditioned on $x_1,...,x_{i-1}, t$, $tT_i(x_1,...,x_i)$ and $(1-t)x_i$ are increasing functions in $x_i$ and since both are invertible in $x_i$, we see $G_i^{-1}[x_1,...,x_{i-1},t](x_i)$ exists. 
	Indeed, when $x_i < \epsilon$, \textbf{Step 1} shows we can write
	$$G_i(x_1,...,x_i,t) = tc_i(x_1,...x_{i-1})x_i + (1-t)x_i = (tc_i(x_1,...,x_{i-1}) + 1-t)x_i,$$
	and it follows that $G_i^{-1}[x_1,...,x_{i-1},t](y_i) = \frac{y_i}{tc_i(x_1,...,x_{i-1}) + 1-t}$.
	
	
	
	Thus for $F(y_1,...,y_d,s) = [F_1,...,F_d]^T,$ by a technical lemma below about inversion of triangular velocity fields (Lemma.\ref{lemma:triangularinverse}\todo{format}, we can compute each of its component recursively, where $F_1(y_1,s) = y_1$, and 
	$$F_i(y_1,...,y_i, s) = \frac{y_i}{sc_i(F_1,F_2,...,F_{i-1}) + 1-s}, \forall i, 2\leq i \leq d.$$
	
	Since $c_i\in C^k([0,1]^i)$ and is bounded from below, it follows from a recursive argument that $\frac{F_i(y_1,...y_i,s)}{y_i}\in C^k([0,1]^i\times[0,1])$ and we can write $F_i(y_1,...y_i, s) = c_i'(y_1,...y_{i-1}, s)y_i$ for some function $c_i'\in C^k([0,1]^i\times[0,1]).$
	
	Note $F_i(y_1,...y_i,s) = c_i'(y_1,...y_{i-1},s)y_i$ and $c_i'$ is a continuous function on bounded domain, by choosing $y_i$ sufficiently small, we get $|F_i| < \epsilon$. 
	
	
	Therefore, by the explicit expression for the velocity field \ref{eq:fexpl}\todo{format} and \textbf{Step 1}, we can write the $i$-th component of $f^\Delta(y_1,...y_d, s)$, as 
	\begin{align*}
		&[f_{p_0}^\Delta]_i(y_1,..,y_i,s) = T_i(F(y_1,...,y_d,s)) - F_i(y_1,...y_d,s)\\
		&= T_i(F_1,...F_i) - F_i = c_i(F_1,...F_{i-1})F_i - F_i\\
		&= c_i(F_1,...F_{i-1})c_i'(y_1,...y_{i-1},s)y_i - c_i'(y_1,...y_{i-1},s)y_i\\
		&= (c_i(F_1,...F_{i-1})-1)c_i'(y_1,...y_{i-1},s)y_i.  \\
	\end{align*}
	
	It follows that 
	$[g^\Delta_{p_0}]_i = \frac{[f_{p_0}^\Delta]_i(y_1,..,y_i, s)}{y_i}\in C^k([0,1]^i\times[0,1]$ for all $i\in\{1,2,...,d\}$ and $y_i\in [0,\epsilon]$. By a similar argument, we can also show $[g^\Delta_{p_0}]_i = \frac{[f_{p_0}^\Delta]_i(y_1,..,y_i, s)}{(1-y_i)}\in C^k([0,1]^i\times[0,1])$ for all $i\in\{1,2,...,d\}$ and $y_i\in[1-\epsilon,1]$. 
	
	\textbf{Step 3: Conclude that $f^\Delta_{p_0}\in\mathcal{V}$}
	
	Observe that the outnormal vectors along the boundary of a $d-$dimensional unit cube are just the standard basis vectors $e_1,..e_d$ where $e_i$ is one in the $i-$th coordinate and zero elsewhere.  Let $\nu = e_i$ for some $i$. Then $f^\Delta_{p_0}\cdot\nu = (f^\Delta_{p_0}(y_1,..,y_i, s)_{i}.$ Near the boundary which $\nu$ is outnormal to, $y_i$ is close to zero or one. Without loss of generality, we may just assume that $y_i\leq\epsilon$ for $\epsilon$ small enough. Then by the linear-vanishing property shown in \textbf{Step 2}, we can write $[f^\Delta_{p_0}]_{i}$ as a product of a $C^k$ function in $y_1,..y_{i-1}, s$ with $y_i$, which approaches zero as $y_i$ approaches zero. Since this holds for all $i$, we can conclude that $f\cdot\nu \equiv 0$ on $\partial D$ 
	
\end{proof}

For the preceding proof, we have used the 

\begin{lemma}\label{lemma:triangularinverse}
	Let $H:[0,1]^d\to[0,1]^d$ be a bijective triangular vector field, i.e., we can write $H(x_1,...,x_d) = [H_1(x_1),...,H_d(x_1,...,x_d)]^T$ where each $H_i(x_1,...x_i): [0,1]^i\mapsto [0,1]$ is a scalar field. Suppose that in each $H_i$, the inverse in the last coordinate while treating all the previous $i-1$ components as fixed, exists. Denote these inverses by $$H_i^{-1}[x_1,...x_{i-1}]: y\mapsto H_i(x_1,...x_{i-1},y).$$
	
	Then, for $y\in [0,1]^d$, we can explicitly write the inverse field $H^{-1}$ using these partial inverses as follows: 
	$$H^{-1}(y_1,y_2,...,y_d) = [h_1, h_2,....h_d],$$
	where 
	$h_1 = H_1^{-1}(y_1), h_2 = H_2^{-1}[h_1](y_2),..., h_d = H_d^{-1}[h_1,...h_{d-1}](y_d)$. 
\end{lemma}
\begin{proof}
	The proof is a direct calculation component by component:
	$$H^{-1}(H(x_1,...x_d))_1 = H_1^{-1}(H_1(x_1)) = x_1.$$
	
	Suppose we've computed components up to $i-1$ for any $2 \leq i \leq d$, then,
	$$H^{-1}(H(x_1,...x_d))_i = H_i^{-1}[x_1,...x_{i-1}](H_i(x_1,...x_i)) = x_i,$$
	where the last equality follows from the definition of $H_i^{-1}[x_1,...x_{i-1}]$. 
	
	The other direction $H(H^{-1}(y_1,...,y_d)) = [y_1,..,y_d]^T$ can be shown in a similar fashion and we omit the computations here. 
\end{proof}






  suffices that $f(x)$
    Consider $\tilde f(x):=\frac{f(x_1/2,x_2,\dots,x_d)}{1-x_1/2}$.
    Then $\tilde f\in C^n(D)$ satisfies the assumptions of Lemma
    \ref{lemma:hardy1} and we find that
    $\tilde g(x)=\frac{f(x_1/2,x_2,\dots,x_d)}{x_1/2(1-x_1/2)}$
    belongs to $C^n(D)$ with its norm bounded by
    \begin{equation*}
      C\norm[C^n(D)]{\partial_{x_1}\tilde f}
      \le C \norm[{C^n([0,1/2]\times [0,1]^{d-1})}]{\partial_{x_1}\frac{f(x)}{1-x_1}}\le \tilde C
      \norm[{C^n([0,1/2]\times [0,1]^{d-1})}]{\partial_{x_1}f(x)},
    \end{equation*}
    for some $\tilde C$ independent of $f$. Since
    \begin{equation*}
      \norm[{C^n([0,1/2]\times [0,1]^{d-1})}]{\frac{f(x)}{x_1(1-x_1)}}
      \le 2^n
      \norm[{C^n(D)}]{\tilde g}
    \end{equation*}
    we find the required bound on $[0,1/2]\times [0,1]^{d-1}$.
    By symmetry this concludes the proof.
  \end{proof}

==> old-abstract.tex <==
\begin{abstract} Differential equations provide a framework to represent invertible transformations of measures, which are recently%
used extensively to represent complex
probability distributions (e.g., in generative modelling and density estimation). While such models have achieved enormous
  success in machine learning and data science, little is known about
  their statistical properties. In this work, we first establish a
  general statistical convergence theorem for distribution learning
  via ODE-parameterized transport maps that is applicable to any
  velocity field class $\mathcal{F}$ satisfying certain simple
  constraints. The proof of this general theorem combines analytical
  stability estimates of ODEs with classical empirical process theory
  for sieved M-estimators. Subsequently, we specialize the general
  theorem to $C^k$-smooth densities. We show the velocity field
  inherits the regularity from the target density, which enables
  considering estimation over a $C^k$ ball and obtaining concrete
  minimax convergence rate. Finally, we consider the setting of neural
  differential equations (neural ODEs), where $\mathcal{F}$ is
  parameterized by a neural network class. Applying our general
  theorem with classical NN approximation results and metric entropy
  rates, we obtain minimax convergence rates and show how the network
  size (e.g., width, depth, sparsity and norm constraints) should
  scale with sample size $n$.\ymtd{make some edits here}
  
\end{abstract}

